epBRM: Improving a Quality of 3D Object Detection using End Point Box Regression Module

We present an endpoint box regression module(epBRM), which is designed for predicting precise 3D bounding boxes using raw LiDAR 3D point clouds. The proposed epBRM is built with sequence of small networks and is computationally lightweight. Our approach can improve a 3D object detection performance by predicting more precise 3D bounding box coordinates. The proposed approach requires 40 minutes of training to improve the detection performance. Moreover, epBRM imposes less than 12ms to network inference time for up-to 20 objects. The proposed approach utilizes a spatial transformation mechanism to simplify the box regression task. Adopting spatial transformation mechanism into epBRM makes it possible to improve the quality of detection with a small sized network. We conduct in-depth analysis of the effect of various spatial transformation mechanisms applied on raw LiDAR 3D point clouds. We also evaluate the proposed epBRM by applying it to several state-of-the-art 3D object detection systems. We evaluate our approach on KITTI dataset, a standard 3D object detection benchmark for autonomous vehicles. The proposed epBRM enhances the overlaps between ground truth bounding boxes and detected bounding boxes, and improves 3D object detection. Our proposed method evaluated in KITTI test server outperforms current state-of-the-art approaches.

==> figures/dist_bound.tex <==
% This file was created by matplotlib2tikz v0.6.18.
\begin{tikzpicture}

\begin{axis}[
axis on top,
height=5.0cm,
legend cell align={left},
legend columns=3,
legend entries={{PointPillars},{F-PointNet},{AVOD(FPN)}},
legend style={at={(0.5,1.2)}, anchor=north, draw=none},
tick pos=both,
width=8.3cm,
xlabel={$dist_{\text{bound}} (m)$},
xmajorgrids,
xmin=-0.03, xmax=0.45,
ylabel={ratio (\%)},
ymajorgrids,
ymin=60, ymax=80
]
\addlegendimage{no markers, blue}
\addlegendimage{no markers, green!50.0!black}
\addlegendimage{no markers, red}
\addplot [line width=1.2400000000000002pt, blue, mark=*, mark size=2, mark options={solid,draw=none}]
table [row sep=\\]{%
0	73.37 \\
0.05	74.34 \\
0.1	75.85 \\
0.15	76.62 \\
0.2	76.2 \\
0.25	75.52 \\
0.3	75.56 \\
0.35	73.96 \\
0.4	72.61 \\
};
\addplot [line width=1.2400000000000002pt, green!50.0!black, mark=square*, mark size=2, mark options={solid,draw=none}]
table [row sep=\\]{%
0	62.79 \\
0.05	63.75 \\
0.1	64.6 \\
0.15	65.44 \\
0.2	65.7 \\
0.25	65.36 \\
0.3	65.99 \\
0.35	65.26 \\
0.4	64.16 \\
};
\addplot [line width=1.2400000000000002pt, red, dashed, mark=square*, mark size=2, mark options={solid,draw=none}]
table [row sep=\\]{%
0	65.8 \\
0.05	66.31 \\
0.1	67.45 \\
0.15	68.24 \\
0.2	67.49 \\
0.25	67.38 \\
0.3	67.42 \\
0.35	66.17 \\
0.4	65.37 \\
};
\addplot [line width=1.2400000000000002pt, black, opacity=0.5, dashed, forget plot]
table [row sep=\\]{%
0.145	60 \\
0.145	80 \\
};
\addplot [line width=1.2400000000000002pt, black, opacity=0.5, dashed, forget plot]
table [row sep=\\]{%
0.155	60 \\
0.155	80 \\
};
\addplot [line width=1.2400000000000002pt, black, opacity=0.5, dashed, forget plot]
table [row sep=\\]{%
0.295	60 \\
0.295	80 \\
};
\addplot [line width=1.2400000000000002pt, black, opacity=0.5, dashed, forget plot]
table [row sep=\\]{%
0.305	60 \\
0.305	80 \\
};
\end{axis}

\end{tikzpicture}
